PushdownDB: Accelerating a DBMS using S3 Computation

This paper studies the effectiveness of pushing parts of DBMS analytics queries into the Simple Storage Service (S3) engine of Amazon Web Services (AWS), using a recently released capability called S3 Select. We show that some DBMS primitives (filter, projection, aggregation) can always be cost-effectively moved into S3. Other more complex operations (join, top-K, group-by) require reimplementation to take advantage of S3 Select and are often candidates for pushdown. We demonstrate these capabilities through experimentation using a new DBMS that we developed, PushdownDB. Experimentation with a collection of queries including TPC-H queries shows that PushdownDB is on average 30% cheaper and 6.7X faster than a baseline that does not use S3 Select.

==> discussion.tex <==
% !TEX root =  main.tex

\section{Limitation of S3 Select} \label{sec:discussion}
\vspace{-.1in}

So far, we have demonstrated substantial performance improvement on common database operators by leveraging S3 Select. 
%We have also discovered various limitations of the current S3 Select features that constrain further performance improvement. 
In this section, we present a list of limitations of the current S3 Select features and describe our suggestions for further improvement. 

\textbf{Suggestion 1: Multiple byte ranges for GET request.}
The indexing algorithm discussed in Section~\ref{ssec:indexing} sends HTTP GET requests to S3 to load records from the table; each request asks for a specified range of bytes that are derived from an index table lookup. According the S3's API~\cite{get-object}, the current GET request to S3 supports only a single byte range. 
This means that a large number of GET requests 
have to be sent if many records are selected by a query. Excessive GET requests can hurt performance as shown in Figure~\ref{fig:filter}. 
Allowing a single GET request to contain multiple ranges can significantly reduce the cost of HTTP request processing in both the server and S3.


\textbf{Suggestion 2: Index inside S3.}
A more thorough solution to the indexing problem is to build the index structures entirely inside S3. 
This avoids multiple rounds of network messages between S3 and the server that are caused by accesses to the index data structure during an index lookup. 
S3 can handle the required logic on behalf of the server, like handling hash collisions in a hash index or traversing through the tree in a B-tree index.

\textbf{Suggestion 3: More efficient Bloom filters.}
Bloom filters can substantially improve performance of join queries, as demonstrated in Section~\ref{sec:join}. 
A Bloom filter is represented using a bit array for space efficiency. 
The current S3 Select, however, does not support bit-wise operators. 
Our current implementation of a Bloom join in S3 Select uses a string of 0’s and 1’s to represent the bit array, which is space- and computation-inefficient. 
We suggest the next version of S3 Select should support efficient bit-wise operators to improve the efficiency of Bloom join.


\textbf{Suggestion 4: Partial group-by.}
Section~\ref{sec:hybrid-groupby} demonstrated the superior performance of the hybrid group-by algorithm. However, since S3 does not currently support group-by queries, we used the \texttt{CASE} clause to implement S3-side group-by, which is not the most efficient implementation. We suggest adding partial group-by queries to S3 to resolve this performance issue. Note that pushing an arbitrary group-by query entirely to S3 may not be the best solution, because a large number of groups can consume significant memory space and computation in S3. We consider the partial S3-side group-by as an optimization to the second phase of our current hybrid group-by.



\textbf{Suggestion 5: Computation-aware pricing.}
Across our evaluations on the optimized \name, S3 Select data scan costs dominate a majority of queries. In the current S3 Select pricing model, data scanning costs a fixed amount (\$0.002/GB) regardless of what computation is being performed. 
Given that our queries typically require very little computation in S3, the current pricing model may have substantially overcharged our queries. 
We believe a fairer pricing model is needed, in which the data scan cost should depend on the workload.

\vspace{-.1in}
